What goes on inside rumour and non-rumour tweets and their reactions: A Psycholinguistic Analyses

In recent years, the problem of rumours on online social media (OSM) has attracted lots of attention. Researchers have started investigating from two main directions. First is the descriptive analysis of rumours and secondly, proposing techniques to detect (or classify) rumours. In the descriptive line of works, where researchers have tried to analyse rumours using NLP approaches, there isnt much emphasis on psycho-linguistics analyses of social media text. These kinds of analyses on rumour case studies are vital for drawing meaningful conclusions to mitigate misinformation. For our analysis, we explored the PHEME9 rumour dataset (consisting of 9 events), including source tweets (both rumour and non-rumour categories) and response tweets. We compared the rumour and nonrumour source tweets and then their corresponding reply (response) tweets to understand how they differ linguistically for every incident. Furthermore, we also evaluated if these features can be used for classifying rumour vs. non-rumour tweets through machine learning models. To this end, we employed various classical and ensemble-based approaches. To filter out the highly discriminative psycholinguistic features, we explored the SHAP AI Explainability tool. To summarise, this research contributes by performing an in-depth psycholinguistic analysis of rumours related to various kinds of events.

==> Introduction_old.tex <==
\section{Introduction}
\fixme{\begin{enumerate}
    \item Let us not bring Fake news, we only stick to rumours. \sabur{removed}
    \item Concluding para of Section 5 is missing. Table 3 can be used for concluding para. \sabur{added}
\end{enumerate}}
%Write a paragraph on Rumour detection
The credibility of information is the most decisive issue on social media. Unmoderatted nature of social media text has resulted in several cases of rumour spreading~\cite{derczynski2017semeval}. Scientific studies to understand the malicious intentions of spreading fake news through the psychological processes involved in the use of language can help in textual classification and behaviour analyses of users. Despite this apparent robustness of social media, its increasing tendency to give rise to rumours~\footnote{Rumour is an unproven statement that is initiated from different sources and disseminates periodically from one point to another point in a network}\fixme{\sout{add a footnote and write definition of rumour?}} motivates the development of systems that, by gathering and analysing the collective judgements of users~\cite{lukasik2016hawkes}, are able to reduce the spread of rumours by accelerating the sense-making process~\cite{derczynski2014pheme}. Hence, linguistics and natural language processing researchers have taken the onus to study how users have discussed rumours and to understand the psycho-linguistic attributes connected to rumour spreading and detection~\cite{ giachanou2021detection, shu2019defend}. 

It has been established that \say{rumours may spread misinformation or disinformation, which are forms of false information~\cite{qazvinian2011rumor, vosoughi2017rumor}}. %\fixme{Raj: \sout{Just 1 definition would do. If we need space, we can remove 2 out of 3.}}
\fixme{Previously we defined 3 definitions of rumour and suddenly classification? I think flow issues} Many of the approaches for rumour detection, use linguistic and psycho-linguistic features for classification~\cite{vosoughi2018spread, giachanou2019leveraging}. Psycho-linguistic in general tell us about the  mutual relationship between human mind and the language. Meanwhile, linguistic attributes tend to convey meaning about the naturally occurring user behaviours and beliefs. Through text analyses, one can determine what a person is trying to convey to another person or group. However the patterns in linguistic behaviour cannot be determined in individual instances and need to have aggregated supervised data processed by computing psycho-linguistic methods and statistical evidences.  

Over the decade, we have seen increasing methods using a variety of machine learning and deep learning techniques to achieve effective accuracies~\cite{ma2018rumor, geng2019rumor}. For example, for the early detection of rumours traditional handcrafted features have been used~\cite{nguyen2017comprehensive}. The authors used two approaches including neural network-based hidden representation of individual author-related text and handcrafted features. The credibility of the tweets is tested in two steps, first event-related data is extracted and tweets are identified as credible with the help of a separate pre-trained model and in the second step, the pipeline features are added to the credit score in a time series based feature vector to identify the rumour tweets. However, these methods and features are unable to answer "why" a piece of text has been classified a certain way. \fixme{suggestion - In this work, we use  Psycho-linguistic analysis for answering "Why"?}

\fixme{Next para -- suggestion for adding text from above para here --  Psycho-linguistic in general tell us about the  mutual relationship between human mind and the language. Meanwhile, linguistic attributes tend to convey meaning about the naturally occurring user behaviours and beliefs. Through text analyses, one can determine what a person is trying to convey to another person or group. However the patterns in linguistic behaviour cannot be determined in individual instances and need to have aggregated supervised data processed by computing psycho-linguistic methods and statistical evidences.  
}
In the article, we investigate the following research questions:

\textbf{RQ 1:} Is there a difference in psycho-linguistic characteristics between rumour and non-rumour source tweets?

\textbf{RQ 2:} How can psycho-linguistic features be used to differentiate between the reactions that rumour and non-rumour tweets attract? 

%\sout{What does the psycho-linguistic features tell us about the characteristics and mindset of the fake news propagator on social media?}


\textbf{RQ 3:} Does the contribution of psycho-linguistic features vary from event to event or do they remain consistent for all events?



%What can we learn about the reaction tweets of rumour and non-rumour tweets?

\textbf{RQ 4:} Can we exploit these features for classifying rumour and non-rumour tweets using Machine Learning models?
%Can we exploit psycho-linguistic features for identifying rumours and non-rumours text and their reactions? 

%\sout{Are machine learning models reliable to identify rumours and non-rumours tweets using psycho-linguistic analysis}
%\fixme{\sout{suggestion for the previous line. I prefer to use psycho-linguistic the earlier part of the sentence. This way we are forming uniformity like other sentences -- Can we exploit psycho-linguistic features for identifying rumours and non-rumours TEXT [note TEXT makes sense, as we have not mentioned tweeter at this point?] by using machine learning models?}}

\textbf{RQ 5:} Which psycho-linguistic features are highly discriminative for identifying rumour and non-rumour class for the classification task? 


%\sout{What are the distinct psycho-linguistic features that differentiate rumour tweets from non-rumour tweets? Which feature contributes significantly in which class.}


To answer these research questions we used the most popular PHEME-9 dataset for rumour classification and divided the dataset based on event. We extracted readability features, emotions, LIWC features and SenticNet features for the psycho-linguistic analyses. All these features gave us more insight and perspective about the mentality of users that are spreading rumours. We calculated the statistical significance and mean values of every psycho-linguistic feature for rumour class, non-rumour class, reactions of rumour tweets and reactions of non-rumour tweets respectively. The statistical analyses helped us derive insights about the personal attributes of the users in these tweets. We further used machine learning classifiers (Random Forest, SVM etc.) on every event to evaluate the robustness of the models in differentiation rumour tweets and their reactions with these features. Lastly, we use SHAP, an explainable machine learning based on shapely values to identify the measure of contributions each feature has in the model. 

Sections 2 sheds light on the related work, while Section 3 and 4 explain the dataset and the methodology. Research findings of RQ1, RQ2 and RQ3 can be seen in Section 5 where we analyzed different features used and how they contributed significantly collectively and separately in each event. We discovered that rumour source tweets use more past related words, prepositions and contains drives (motivation) related to reward, risk and power. Similarly, non-rumour source tweets had more mean of features such as affective processes, cognitive processes (insight, causation, discrepancy, certainty, differentiation), present related words, informal language and had drives related to affiliation and achievement. A detailed analyses of that is shown in Table~\ref{tbl:featurepartition}. Findings of RQ4 and RQ5 can be found in Section 6 where we discussed the results of the machine learning models and explained the SHAP plots for rumour and non-rumour tweets. We discovered that different features contribute in the classification of both rumour tweets and their reactions i.e fear and function words in the rumour class. For a more  visual explanation we refer you to Figure~\ref{subfig-2:shap_reply} and Table~\ref{tbl:prediction-results}. Finally, Section 6 gives the conclusion of the findings in the article. 

%\fixme{\sout{I am bit confused about the objective of this work. We are discussing about " derive insights about the personal attributes of the users in these tweets". This seems cherry on the cake? It might gave an impression that we are more interested in "what is going inside the mind of users involved in the mind of rumour spreaders.}}


\fixme{\begin{enumerate}
    \item What is the objective of this work
    \item Short summary of what others did in this field (1 paragraph about similar and closed works)
    \item Motivation behind it == Why it is important?
    \item What we did: Dataset, methodology and results. Results can be shown as a contribution? For example, -- To the best of our knowledge we are showing through "Psycholinguistic Analyses" interpretability?
    \item We should say -- every news item , rumour and non-rumour attracts reaction. Whether it is like DEFEND paper (or some others) which have analysed news and comments. Here, we are analysing that model using Twitter and its retweets using a public dataset.
    \item Future work- we need to run it on bigger text (like news item)
    \item Some possible interesting results that we should mention in the introduction are the following:
    \begin{enumerate}
        \item The statistics show how source tweets needed more convincing and engagement and also engaged more non-rumoured reply tweets to deny the rumoured claims
    \end{enumerate}
\end{enumerate}}



\begin{comment}
\begin{table}[]
\caption{The table shows the partition of features according to categories based on mean and statistical significance}
\resizebox{\columnwidth}{!}
  {%
\label{tab:featurepartition}
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \textbf{Higher mean in Rumour}                                                                                                                                             & \multicolumn{1}{c|}{\textbf{Higher mean in Non-Rumour}}                                                                                                                                    \\ \hline
\textbf{Source tweets} & \begin{tabular}[c]{@{}c@{}}- Use of prepositions \\ - Social words (family)\\ - Cognitive Processes (tentative)\\ - Time (Past)\\ - Relativity\\ - Personal (work, death, leisure)\\ - Drives (reward, risk,  power)\\ - SenticNet (pleasantness, attention, polarity)\\ - Emotions (fear, sadness)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}- Average Word count\\ - Personal Pronouns (1st person singular (I), 1st person plural (we), \\ 2nd person(you), 3rd person singular (S/he \textbackslash{}fixme\{\textbackslash{}sout\{S/he\}\}) , \\ 3rd person plural (they))\\ - Conjunction, common adverbs, auxiliary verbs\\ - Affective processes\\ - Cognitive Processes (insight, causation, discrepancy, certainty, differentiation)\\ - Time (Present)\\ - Personal (home, money, religion)\\ - Informal language\\ - Drives (affiliation, achievement)\\ - Grammar (interrogative, comparison)\\ - SenticNet (sensitivity)\\ - Emotions (Neutral, fear, anger)\end{tabular}} \\ \hline
\textbf{Reactions}     & \begin{tabular}[c]{@{}c@{}}Negation words\\ - Cognitive Processes (tentative)\\ - Time (Past)\\ - Relativity\\ - Emotions (anger, surprise)\end{tabular}                                                                                                                                                         & \begin{tabular}[c]{@{}c@{}}- Personal pronouns \\ - Impersonal pronouns, auxiliary verbs, conjunctions \\ - Negation words\\ - Affective processes\\ - Cognitive Processes (insight, causation, discrepancy, certainty, differentiation)\\ - Time (Present)\\ - Grammar (interrogative, comparison)\\ - SenticNet (pleasantness, sensitivity)\\ - Emotions (fear)\end{tabular}                                                                                                                                                                                                                                                                                                           \\ \hline
\end{tabular}
}
\end{table}
\end{comment}


%\begin{enumerate}
%    \item \textbf{How do we know how people are reacting to the the rumours? Is it different}
%\item \textbf{Mention how datasets are balanced in the scenario}
%\item \textbf{Mention how reactions can be used in other scenarios, is it %possible?}
%\item \textbf{How this study can benefit other studies in rumour/fake}
%\item manipulate human mind, what are they trying to achieve
%\end{enumerate}

%\sak{Suggestions for RQs:RQ1. Do psycho-linguistic characteristics have an impact on rumour and non-rumour source tweets?2nd version of RQ1. Is there a difference in psycho-linguistic characteristics between rumour and non-rumour source tweets?RQ2. What effect do these features have on reaction tweets?RQ3. Is the psycho-linguistic contribution vary from one incident to the next, or is it stable across all sorts of rumour?RQ4. Can we exploit these features for classifying rumour and non-rumour tweets using Machine Learning models?RQ5: Can we uncover important traits in discerning between rumour and non-rumour tweets?2nd version of RQ5. Is there any feature in the classification task that is more crucial (useful) than the others?}

==> RWbackup.tex <==
\section{Related Work}
\fixme{Related work is written w.r.t detection/classification of rumours. However, we need papers which more about analysis or at least they should have analysis. Also, I think we should discuss first papers about analysis and then about detection.}
\begin{comment}
\fixme{We need to have following set of papers
\begin{enumerate}
    \item Papers in general about rumours
    \item Papers covering LIWC aspects
    \item Papers about explainability and INterpretability (DEFEND, etc)
    \item Papers closely related to ours. What is the difference between present work and previous works (Which are closely related to us)
\end{enumerate}
}
\end{comment}

Psychological perspectives have been used in several studies to find a correlation with conspiracy theories. Douglas et al.~\cite{douglas2017psychology} wrote extensively on the psychological factors and divided them into existential (e.g. desire for control), social (e.g. desire to maintain a positive image of the self or group) and epistemic (e.g. desire for understanding) factors. The author explained that these factors contribute to the popularity of conspiracy theories. Another study discovered~\cite{lantian2017know} that conspiracies urge from the need for uniqueness. Similarly, in the light of the COVID-19 pandemic, researchers~\cite{callaghan2019parent} have correlated a high level of conspiracy thinking of parents with the delay of vaccination among children. While there are studies that have attempted to discover the correlation of psycholinguistics with fake news~\cite{shu2019defend} and conspiracy~\cite{rains2021psycholinguistic}  in general, we narrowed it down to the understanding of rumour. 



Various NLP studies have been published related to rumour detection in text. %\fixme{Please check next 2 lines.}
These  studies mostly revolve around the data collection, techniques and features suitable for identifying rumour text. Among the components of rumour detection, rumour has been explored~\cite{varshney2020review} in the context of rumour tracking, rumour stance classification, rumour detection, and rumour veracity classification. The Rumour detection task can be topic-level~\cite{yang2015emerging} or post-level~\cite{derczynski2017semeval}, where the task is to identify if the topic is relevant to the text or if the post information has rumour respectively. The trend of rumour detection on topic-level has shifted quickly towards the post level understanding of rumour and, hence, needs insightful analyses for understanding linguistic and psycho-linguistic attributes of rumour. 


Different statistical methods used for rumour detection have used a variety of features~\cite{vosoughi2017rumor, geng2019rumor, jin2017multimodal, yang2015emerging, kwon2013prominent} for social media text as listed below:
\fixme{Can we reuse existing citations for the following enumeration?}
\begin{enumerate}
\item User-based features include verified profile, follower count, number of people following, the time interval of posts, description, number of posts, URL, description etc.  
\item User-behaviour based features include the number of reposts, number of comments per day, average number of followers etc.
\item Linguistic based features include negation words, opinion words, insights, formality and sophistication of tweets.
\item Message-based features include character length, word length, question marks, exclamation marks etc.
\item Content-based features including the count of the hashtag, at the rate sign, sentiment words, word count etc. 
\end{enumerate}


Other than PHEME which is the benchmark dataset for rumour detection and is used for this study, the popular text based datasets include RUMDECT~\cite{ma2016detecting}, SNAP data~\cite{yang2011patterns}, CrisisLexT26~\cite{olteanu2015expect}, MULTI~\cite{jin2017multimodal}, KWON~\cite{kwon2013prominent} and RUMOUREVAL~\cite{derczynski2017semeval}.  For more insight into features and textual datasets for rumour classification, we recommend reading~\cite{varshney2020review}. 

The most commonly used techniques for rumour detection use traditional Machine learning (TML) methods with selective feature engineering, deep learning models (DL) and hybrid models respectively. In the study~\cite{zubiaga2016learning} authors introduced context-aware rumour detection using a sequential classifier to detect rumours from the tweets divided into five news events. In an outbreak of stories, identifying the emergency is also important for the timely detection of credible information. The work~\cite{xia2012information} used an unsupervised algorithm to label the tweets as credible and incredible and identified the urgency of the news verification using supervised machine learning methods and multiple features (content, author, and diffusion). 

Early detection of the rumour is essential to mitigate the harm and the study~\cite{ma2018rumor} segregated the rumours using a propagation tree. They used recursive neural networks to classify the tweets into false rumour, non-rumour, unverified rumour and true rumour. An Recurrent Neural Network (RNN) based aware provenance approach was proposed~\cite{duong2017provenance} combining the textual information and provenance information to enhance the results. To tackle the cases where provenance details were missing, they used a fusion of text and provenance information. Among the machine learning models~\cite{ashraf2021cic, geng2019rumor, jin2017multimodal, sampson2016leveraging} Support vector machine (SVM), Naive Bayes (NB),
Random Forest (RF), Decision Tree (DT), Logistic Regression (LR), and XGBoost have been used repeatedly. Deep learning models (Convolutional neural network (CNN), Long short-term memory (LSTM), Recurrent neural networks (RNN))~\cite{santhoshkumar2020earlier, kotteti2020ensemble, nguyen2017comprehensive} and transformer-based models (XLNet, BERT, RoBERTa, DistilBERT, and ALBERT)~\cite{transformer1, transformer2} have often given the state of the art results in multiple rumour tasks. 


Psycholinguistic features on rumour detection studies have involved the use of Long Short-Term Memory (LSTM) with LIWC features i.e swear words and personal pronouns~\cite{tausczik2010psychological} and emotions~\cite{vosoughi2018spread}. The study~\cite{vosoughi2018spread} showed the existence of false rumours that triggered fear, disgust and surprise in the rumour replies, while,~\cite{giachanou2019leveraging} proposed an LSTM-based model with emotions to check the credibility of articles. The role of user-profiles was evaluated by ~\cite{shu2018understanding} which showed implicit (age, location) and explicit features (follower count, status count) that contributed to fake news.  In addition, they showed how the combination of these features with the psycho-linguistic characteristics (LIWC, Writing styles) can be effective. Another study~\cite{giachanou2020role} proposed a CNN based model combined with personality traits (Big-five) and LIWC to distinguish between fake users.  Similarly, the authors~\cite{giachanou2021detection} gave a comparative analysis over various profile, linguistic and psychological characteristics (Big-five personality traits, LIWC, emotions) and used CNN based classifier with word embeddings and psycho-linguistic characteristics for classification. 

Contrary to these studies, our focus is on the explainability of these features in the context of why these features contribute to the rumour or non-rumour classes as well as their reactions and what does it tell us about the tweets. It should be noted that none of these papers indulges in the explainability aspects of psycholinguistics in rumour tweets and reaction tweets. Also, none of these studies gives an insight into the features comparing different events as every event triggers a different insight. 



==> Tables/LIWC_mean.tex <==
\begin{table}[!htbp]
\begin{tabular}{ccccc}
\textbf{}                                               & \textbf{Rumour Source} & \textbf{Non-rumour Source} & \textbf{Rumour Reaction} & \textbf{Non-Rumour Reaction} \\
\multicolumn{1}{l}{\textbf{Word Count}}                 & 20                     & 20.02                      & 14.63                    & 15.09                        \\
\multicolumn{1}{l}{\textbf{Summary Language Variables}} & -                      & -                          & -                        & -                            \\
\multicolumn{1}{l}{Analytical thinking}                 & 89                     & 82.27                      & 64.19                    & 61.47                        \\
\multicolumn{1}{l}{Clout}                               & 62                     & 61.73                      & 57.75                    & 58.67                        \\
\multicolumn{1}{l}{Authentic}                           & 24                     & 23.78                      & 24.90                    & 23.80                        \\
\multicolumn{1}{l}{Emotional tone}                      & 29                     & 31.01                      & 33.98                    & 36.55                        \\
\multicolumn{1}{l}{Words/sentence}                      & 15                     & 14.67                      & 10.67                    & 10.84                        \\
\multicolumn{1}{l}{Words \textgreater 6 letters}        & 27                     & 26.66                      & 30.08                    & 30.69                        \\
\multicolumn{1}{l}{Dictionary words}                    & 55                     & 57.79                      & 63.36                    & 64.22                        \\
\multicolumn{1}{l}{\textbf{Linguistic Dimensions}}      & -                      & -                          & -                        & -                            \\
\multicolumn{1}{l}{Total function words}                & 24                     & 29.26                      & 33.65                    & 35.10                        \\
Total pronouns                                          & 3                      & 6.06                       & 9.374                    & 10.36                        \\
Personal pronouns                                       & 1                      & 3.20                       & 5.166                    & 6.02                         \\
\multicolumn{1}{r}{1st pers singular}                   & 0                      & 0.85                       & 1.415                    & 1.735                        \\
\multicolumn{1}{r}{1st pers plural}                     & 0                      & 0.89                       & 0.5436                   & 0.671                        \\
\multicolumn{1}{r}{2nd person}                          & 0                      & 0.57                       & 1.38                     & 2.064                        \\
\multicolumn{1}{r}{3rd pers singular}                   & 0                      & 0.31                       & 0.8653                   & 0.5588                       \\
\multicolumn{1}{r}{3rd pers plural}                     & 0                      & 0.48                       & 0.9671                   & 0.9887                       \\
Impersonal pronouns                                     & 1                      & 2.34                       & 4.152                    & 4.265                        \\
Articles                                                & 3                      & 4.08                       & 3.98                     & 3.986                        \\
Prepositions                                            & 11                     & 10.77                      & 7.81                     & 7.828                        \\
Auxiliary verbs                                         & 4                      & 4.71                       & 6.761                    & 7.114                        \\
Common Adverbs                                          & 2                      & 2.35                       & 3.834                    & 3.872                        \\
Conjunctions                                            & 2                      & 2.39                       & 3.007                    & 3.254                        \\
Negations                                               & 1                      & 1.14                       & 2.02                     & 2.111                        \\
\multicolumn{1}{l}{\textbf{Other Grammar}}              & -                      & -                          & -                        & -                            \\
\multicolumn{1}{l}{Common verbs}                        & 8                      & 8.66                       & 12.14                    & 12.49                        \\
\multicolumn{1}{l}{Common adjectives}                   & 3                      & 3.05                       & 3.44                     & 3.578                        \\
\multicolumn{1}{l}{Comparisons}                         & 1                      & 1.41                       & 1.406                    & 1.424                        \\
\multicolumn{1}{l}{Interrogatives}                      & 1                      & 0.92                       & 1.333                    & 1.434                        \\
\multicolumn{1}{l}{Numbers}                             & -                      & -                          & -                        & -                            \\
\multicolumn{1}{l}{Quantifiers}                         & 1                      & 1.04                       & 1.365                    & 1.482                        \\
\multicolumn{1}{l}{\textbf{Psychological Processes}}    & -                      & -                          & -                        & -                            \\
\multicolumn{1}{l}{Affective processes}                 & 3                      & 5.17                       & 7.034                    & 7.624                        \\
Positive emotion                                        & 1                      & 2.16                       & 3.293                    & 3.851                        \\
Negative emotion                                        & 2                      & 3.19                       & 3.735                    & 3.778                        \\
\multicolumn{1}{r}{Anxiety}                             & 0                      & 0.67                       & 0.625                    & 0.598                        \\
\multicolumn{1}{r}{Anger}                               & 1                      & 1.68                       & 1.566                    & 1.744                        \\
\multicolumn{1}{r}{Sadness}                             & 0                      & 0.30                       & 0.5049                   & 0.4208                       \\
\multicolumn{1}{l}{Social processes}                    & 5                      & 6.24                       & 7.793                    & 8.288                        \\
Family                                                  & 0                      & 0.36                       & 0.2591                   & 0.2129                       \\
Friends                                                 & 0                      & 0.23                       & 0.2832                   & 0.2617                       \\
Female references                                       & 0                      & 0.31                       & 0.1743                   & 0.2003                       \\
Male references                                         & 1                      & 0.45                       & 1.197                    & 7.961                        \\
\multicolumn{1}{l}{Cognitive processes}                 & 4                      & 5.44                       & 8.490                    & 9                            \\
Insight                                                 & 1                      & 1.46                       & 1.738                    & 1.699                        \\
Causation                                               & 1                      & 0.89                       & 1.289                    & 1.455                        \\
Discrepancy                                             & 0                      & 0.80                       & 1.163                    & 1.231                        \\
Tentative                                               & 1                      & 0.99                       & 1.841                    & 1.735                        \\
Certainty                                               & 0                      & 0.99                       & 1.374                    & 1.566                        \\
Differentiation                                         & 1                      & 1.50                       & 2.320                    & 2.522                        \\
\multicolumn{1}{l}{Perceptual processes}                & 2                      & 2.15                       & 2.013                    & 2.043                        \\
See                                                     & 1                      & 1.23                       & 0.9938                   & 1.022                        \\
Hear                                                    & 1                      & 0.72                       & 0.6940                   & 0.685                        \\
Feel                                                    & 0                      & 0.26                       & 0.2582                   & 0.2786                       \\
\multicolumn{1}{l}{Biological processes}                & 1                      & 1.06                       & 1.39                     & 1.324                        \\
Body                                                    & 0                      & 0.34                       & 0.5299                   & 0.5051                       \\
Health                                                  & 1                      & 0.35                       & 0.4101                   & 0.3304                       \\
Sexual                                                  & 0                      & 0.10                       & 0.2240                   & 0.2631                       \\
Ingestion                                               & 1                      & 0.26                       & 0.2818                   & 0.1942                       \\
\multicolumn{1}{l}{Drives}                              & 7                      & 7.16                       & 6.726                    & 6.714                         \\
Affiliation                                             & 1                      & 2.09                       & 1.364                    & 1.628                        \\
Achievement                                             & 0                      & 0.63                       & 0.6453                   & 0.7386                       \\
Power                                                   & 5                      & 4                          & 3.381                    & 3.146                        \\
Reward                                                  & 1                      & 0.6                        & 0.9329                   & 0.9154                       \\
Risk                                                    & 1                      & 0.67                       & 0.8250                   & 0.8332                       \\
\multicolumn{1}{l}{Time orientations}                   & -                      & -                          & -                        & -                            \\
Past focus                                              & 3                      & 1.52                       & 2.345                    & 2.005                        \\
Present focus                                           & 5                      & 6.42                       & 8.544                    & 9.179                        \\
Future focus                                            & 1                      & 1.06                       & 1.002                    & 0.9553                       \\
\multicolumn{1}{l}{Relativity}                          & 12                     & 10.49                      & 8.985                    & 7.894                        \\
Motion                                                  & 1                      & 1.41                       & 1.248                    & 1.077                        \\
Space                                                   & 8                      & 6.38                       & 5.195                    & 4.433                        \\
Time                                                    & 3                      & 3.16                       & 2.656                    & 2.530                        \\
\multicolumn{1}{l}{Personal concerns}                   & -                      & -                          & -                        & -                            \\
Work                                                    & 3                      & 2.17                       & 1.675                    & 1.576                        \\
Leisure                                                 & 2                      & 1.37                       & 0.8619                   & 0.8006                       \\
Home                                                    & 0                      & 0.29                       & 0.2545                   & 0.1576                       \\
Money                                                   & 0                      & 0.34                       & 0.4564                   & 0.3719                       \\
Religion                                                & 1                      & 1.28                       & 1.44                     & 1.72                         \\
Death                                                   & 2                      & 0.79                       & 0.8449                   & 0.6320                       \\
\multicolumn{1}{l}{Informal language}                   & 5                      & 5.32                       & 4.051                    & 4.024                        \\
Swear words                                             & 0                      & 0.20                       & 0.7216                   & 0.6710                       \\
Netspeak                                                & 5                      & 5.02                       & 2.598                    & 2.532                        \\
Assent                                                  & 0                      & 0.30                       & 0.8752                   & 0.7711                       \\
Nonfluencies                                            & 0                      & 0.29                       & 0.3695                   & 0.3901                       \\
Fillers                                                 & 0                      & 0.10                       & 0.04520                  & 0.04783                      \\
\multicolumn{1}{l}{\textbf{Punctuations}}               & \multicolumn{1}{l}{-}  & \multicolumn{1}{l}{-}      & \multicolumn{1}{l}{-}    & \multicolumn{1}{l}{-}        \\
Total Punctuations                                      & 31                     & 33.29                      & 42.80                    & 42.77                        \\
\multicolumn{1}{r}{Periods}                             & 8                      & 9.38                       & 8.413                    & 8.494                        \\
\multicolumn{1}{r}{Commas}                              & 2                      & 2.30                       & 1.768                    & 1.974                        \\
\multicolumn{1}{r}{Colons}                              & 2                      & 1.57                       & 1.191                    & 0.7745                       \\
\multicolumn{1}{r}{Semi-Colons}                         & 0                      & 0.43                       & 0.3027                   & 0.3555                       \\
\multicolumn{1}{r}{Question marks}                      & 0                      & 0.35                       & 1.98                     & 1.779                        \\
\multicolumn{1}{r}{Apostrophes}                         & 1                      & 1.83                       & 2.127                    & 2.361                        \\
\multicolumn{1}{r}{Parentheses}                         & 0                      & 0.33                       & 0.3002                   & 0.2887                       \\
\multicolumn{1}{r}{Other punctuation}                   & 15                     & 16.24                      & 22.73                    & 23.15                       
\end{tabular}
\end{table}

==> tables_and_figures.tex <==

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{sample-franklin}
  \caption{1907 Franklin Model D roadster. Photograph by Harris \&
    Ewing, Inc. [Public domain], via Wikimedia
    Commons. (\url{https://goo.gl/VLCRBB}).}
  \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

